Disambiguated Node Classification with Graph Neural Networks

Graph Neural Networks (GNNs) have demonstrated significant success in learning from graph-structured data across various domains. Despite their great successful, one critical challenge is often overlooked by existing works, i.e., the learning of message propagation that can generalize effectively to underrepresented graph regions. These minority regions often exhibit irregular homophily/heterophily patterns and diverse neighborhood class distributions, resulting in ambiguity. In this work, we investigate the ambiguity problem within GNNs, its impact on representation learning, and the development of richer supervision signals to fight against this problem. We conduct a fine-grained evaluation of GNN, analyzing the existence of ambiguity in different graph regions and its relation with node positions. To disambiguate node embeddings, we propose a novel method, {\method}, which exploits additional optimization guidance to enhance representation learning, particularly for nodes in ambiguous regions. {\method} identifies ambiguous nodes based on temporal inconsistency of predictions and introduces a disambiguation regularization by employing contrastive learning in a topology-aware manner. {\method} promotes discriminativity of node representations and can alleviating semantic mixing caused by message propagation, effectively addressing the ambiguity problem. Empirical results validate the efficiency of {\method} and highlight its potential to improve GNN performance in underrepresented graph regions.

==> secs/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    Yes
  \item Did you describe the limitations of your work?
    Yes
  \item Did you discuss any potential negative societal impacts of your work?
    No
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    Yes
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    n/a
        \item Did you include complete proofs of all theoretical results?
    n/a
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    No
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    Yes
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    Yes
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    No
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    Yes
  \item Did you mention the license of the assets?
    n/a
  \item Did you include any new assets either in the supplemental material or as a URL?
    No
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    N/a
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    n/a
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    n/a
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    n/a
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    n/a
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/hetero_result.tex <==
\begin{table*}
\tiny
  \caption{Results in node classification on three heterophily graph datasets.
  } \label{tab:hetero_result}
  \centering
  \vskip -1em
  \resizebox{0.9\linewidth}{!}{
  \begin{tabular}{ c ccc ccc ccc }
    \toprule
    \multirow{2}*{Method}  & \multicolumn{3}{c}{Squirrel} & \multicolumn{3}{c}{Chameleon} & \multicolumn{3}{c}{Actor} \\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    & ACC & MacroF & AUROC & ACC & MacroF & AUROC & ACC & MacroF & AUROC \\
    \midrule
      SRGNN & $55.9_{\pm 1.4}$ & $56.1_{\pm 1.8}$ & $78.2_{\pm 0.8}$ & $54.1_{\pm 1.9}$ & $55.6_{\pm 1.6}$ & $83.1_{\pm 0.8}$ &   $50.5_{\pm 1.8}$ & $48.1_{\pm 1.3}$ & $85.4_{\pm 0.9}$ \\
      DropEdge & $57.3_{\pm 1.6}$ & $56.7_{\pm 1.7}$ & $78.7_{\pm 0.9}$ & $53.7_{\pm 2.1}$ & $55.3_{\pm 1.5}$ & $83.0_{\pm 0.8}$ &   $51.3_{\pm 1.1}$ & $48.9_{\pm 1.2}$ & $86.3_{\pm 0.8}$ \\
      Focal & $54.7_{\pm 2.1}$ & $55.2_{\pm 2.3}$ & $78.1_{\pm 0.9}$ & $53.3_{\pm 2.5}$ & $54.7_{\pm 1.7}$ & $82.4_{\pm 1.3}$ &   $50.9_{\pm 1.2}$ & $48.7_{\pm 1.4}$ & $85.6_{\pm 0.6}$\\
      ReNode &  $56.3_{\pm 1.8}$ & $56.6_{\pm 1.9}$ & $78.8_{\pm 1.0}$ & $54.3_{\pm 1.7}$ & $55.7_{\pm 1.7}$ & $83.1_{\pm 0.9}$ &   $51.4_{\pm 1.8}$ & $48.8_{\pm 1.6}$ & $85.9_{\pm 1.1}$  \\
      TopoImb & $57.1_{\pm 1.5}$ & $56.8_{\pm 1.5}$ & $79.1_{\pm 0.3}$ & $54.5_{\pm 2.2}$ & $56.1_{\pm 1.4}$ & $82.8_{\pm 0.8}$ &   $51.3_{\pm 1.5}$ & $48.3_{\pm 1.5}$ & $85.9_{\pm 0.8}$ \\
      \midrule
      CE & $56.8_{\pm 1.6}$ & $56.3_{\pm 1.6}$ & $78.4_{\pm 0.6}$ & $53.6_{\pm 2.3}$ & $55.3_{\pm 1.7}$ & $82.9_{\pm 0.9}$ &   $50.8_{\pm 1.4}$ & $48.5_{\pm 1.2}$ & $85.6_{\pm 0.7}$ \\
      + {\method} & $\bm{57.6}_{\pm 1.7}$ & $\bm{57.2}_{\pm 1.4}$ & $79.5_{\pm 0.7}$ & $55.6_{\pm 1.9}$ & $56.4_{\pm 1.4}$ & $83.2_{\pm 0.4}$ &   $51.9_{\pm 1.1}$ & $49.1_{\pm 2.5}$ & $87.7_{\pm 0.4}$ \\
      \midrule
      SupCon & $55.4_{\pm 1.9}$ & $55.2_{\pm 1.7}$ & $77.8_{\pm 0.5}$ & $55.7_{\pm 2.1}$ & $55.9_{\pm 1.8}$ & $83.2_{\pm 0.7}$ &   $51.2_{\pm 2.5}$ & $49.7_{\pm 1.2}$ & $86.7_{\pm 0.8}$ \\
      + {\method} & $56.9_{\pm 1.9}$ & $57.1_{\pm 1.6}$ & $78.4_{\pm 0.8}$ & $56.6_{\pm 1.8}$ & $\bm{56.9}_{\pm 1.6}$ & $\bm{83.5}_{\pm 0.5}$ &   $53.2_{\pm 1.6}$ & $\bm{52.3}_{\pm 1.9}$ & $\bm{88.4}_{\pm 0.5}$\\
      \midrule
      DGI &  $53.9_{\pm 2.1}$ & $52.7_{\pm 1.5}$ & $77.6_{\pm 0.5}$ & $53.5_{\pm 2.2}$ & $54.4_{\pm 2.1}$ & $82.3_{\pm 0.7}$ &   $51.9_{\pm 1.7}$ & $49.1_{\pm 1.4}$ & $86.4_{\pm 0.9}$ \\
      + {\method} & $55.7_{\pm 1.6}$ & $56.1_{\pm 1.8}$ & $\bm{80.3}_{\pm 0.6}$ & $\bm{56.7}_{\pm 2.3}$ & $\bm{56.9}_{\pm 1.6}$ & $83.4_{\pm 0.5}$ &   $\bm{53.4}_{\pm 1.6}$ & $51.2_{\pm 2.6}$ & $88.1_{\pm 0.6}$ \\
    \bottomrule
  \end{tabular}}
\end{table*}

==> tables/main_result.tex <==
\begin{table*}[t]
  \caption{Results in node classification on three benchmark datasets.
  } \label{tab:main_result}
  \centering
  \vskip -1em
  \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{ c ccc ccc ccc }
    \toprule
    \multirow{2}*{Method}  & \multicolumn{3}{c}{Cora} & \multicolumn{3}{c}{BlogCatalog} & \multicolumn{3}{c}{Computer} \\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    & ACC & MacroF & AUROC & ACC & MacroF & AUROC & ACC & MacroF & AUROC \\
    \midrule
      SRGNN & $80.5_{\pm 1.5}$ & $79.6_{\pm 1.7}$ & $89.3_{\pm 0.9}$ & $45.7_{\pm 2.2}$ & $45.1_{\pm 1.6}$ & $82.0_{\pm 1.4}$ &   $76.2_{\pm 1.3}$ & $75.8_{\pm 2.3}$ & $86.8_{\pm 0.7}$ \\
      DropEdge &  $81.1_{\pm 1.5}$ & $80.2_{\pm 1.1}$ & $89.6_{\pm 0.7}$ & $45.5_{\pm 1.8}$ & $45.2_{\pm 1.6}$ & $82.2_{\pm 1.2}$ &   $75.9_{\pm 1.7}$ & $75.9_{\pm 2.6}$ & $86.9_{\pm 0.6}$  \\
      Focal & $80.9_{\pm 1.3}$ & $79.8_{\pm 1.6}$ & $89.6_{\pm 0.7}$ & $45.2_{\pm 2.1}$ & $44.6_{\pm 1.7}$ & $81.7_{\pm 1.5}$ &   $77.3_{\pm 1.9}$ & $75.7_{\pm 2.1}$ & $87.0_{\pm 0.5}$ \\
      ReNode & $81.4_{\pm 1.6}$ & $80.6_{\pm 1.8}$ & $89.7_{\pm 0.6}$ & $45.9_{\pm 2.3}$ & $45.6_{\pm 1.5}$ & $82.7_{\pm 1.3}$ &   $77.1_{\pm 1.5}$ & $75.6_{\pm 2.1}$ & $86.6_{\pm 0.7}$ \\
      TopoImb & $80.6_{\pm 1.7}$ & $79.3_{\pm 1.9}$ & $89.5_{\pm 1.1}$ & $46.1_{\pm 1.8}$ & $45.6_{\pm 1.9}$ & $82.1_{\pm 1.1}$ &   $77.4_{\pm 1.9}$ & $75.9_{\pm 1.9}$ & $87.1_{\pm 0.5}$ \\
      \midrule
      CE & $80.8_{\pm 1.2}$ & $79.9_{\pm 1.5}$ & $89.8_{\pm 0.8}$ & $45.3_{\pm 2.1}$ & $44.8_{\pm 1.8}$ & $81.9_{\pm 1.3}$ &   $76.9_{\pm 1.6}$ & $75.5_{\pm 2.4}$ & $86.7_{\pm 0.6}$ \\
      + {\method} & $81.5_{\pm 1.3}$ & $\bm{81.0}_{\pm 1.4}$ & $89.7_{\pm 0.6}$ & $47.2_{\pm 2.2}$ & $47.6_{\pm 1.3}$ & $\bm{85.3}_{\pm 0.5}$ &   $78.3_{\pm 1.5}$ & $76.3_{\pm 2.3}$ & $87.4_{\pm 0.4}$ \\
      \midrule
      SupCon & $80.6_{\pm 1.5}$ & $79.7_{\pm 1.7}$ & $89.7_{\pm 0.9}$ & $46.5_{\pm 2.3}$ & $46.2_{\pm 1.8}$ & $82.5_{\pm 1.6}$ &   $78.7_{\pm 1.3}$ & $77.1_{\pm 1.9}$ & $88.7_{\pm 0.7}$ \\
      + {\method} & $\bm{81.7}_{\pm 1.4}$ & $80.9_{\pm 1.6}$ & $\bm{89.8}_{\pm 0.5}$ & $\bm{48.6}_{\pm 1.9}$ & $48.5_{\pm 1.2}$ & $84.9_{\pm 0.6}$ &   $\bm{80.1}_{\pm 1.7}$ & $\bm{79.6}_{\pm 2.5}$ & $\bm{89.3}_{\pm 0.5}$ \\
      \midrule
      DGI & $80.7_{\pm 1.9}$ & $79.6_{\pm 2.0}$ & $89.8_{\pm 0.8}$ & $45.9_{\pm 1.8}$ & $46.4_{\pm 2.2}$ & $82.7_{\pm 1.3}$ &   $78.8_{\pm 1.4}$ & $74.7_{\pm 2.4}$ & $88.8_{\pm 0.6}$ \\
      + {\method} & $81.3_{\pm 1.2}$ & $80.3_{\pm 1.5}$ & $89.7_{\pm 0.5}$ & $48.3_{\pm 1.6}$ & $\bm{48.6}_{\pm 1.6}$ & $85.1_{\pm 0.8}$ &   $79.6_{\pm 1.8}$ & $76.5_{\pm 2.2}$ & $89.1_{\pm 0.8}$ \\
    \bottomrule
  \end{tabular}}
\end{table*}
